Mesh-based Dynamics with Occlusion Reasoning for Cloth Manipulation

Self-occlusion is challenging for cloth manipulation, as it makes it difficult to estimate the full state of the cloth. Ideally, a robot trying to unfold a crumpled or folded cloth should be able to reason about the cloth's occluded regions. We leverage recent advances in pose estimation for cloth to build a system that uses explicit occlusion reasoning to unfold a crumpled cloth. Specifically, we first learn a model to reconstruct the mesh of the cloth. However, the model will likely have errors due to the complexities of the cloth configurations and due to ambiguities from occlusions. Our main insight is that we can further refine the predicted reconstruction by performing test-time finetuning with self-supervised losses. The obtained reconstructed mesh allows us to use a mesh-based dynamics model for planning while reasoning about occlusions. We evaluate our system both on cloth flattening as well as on cloth canonicalization, in which the objective is to manipulate the cloth into a canonical pose. Our experiments show that our method significantly outperforms prior methods that do not explicitly account for occlusions or perform test-time optimization. Videos and visualizations can be found on our $\href{https://sites.google.com/view/occlusion-reason/home}{\text{project website}}.$

==> packages.tex <==
% \usepackage{graphics} % for pdf, bitmapped graphics files
% \usepackage{epsfig} % for postscript graphics files
% \usepackage{mathptmx} % assumes new font selection scheme installed
% \usepackage{times} % assumes new font selection scheme installed
% \usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb}  % assumes amsmath package installed
% \usepackage{siunitx} % for SI units
% \usepackage{textcomp}
% \usepackage{gensymb} % for degree command
\usepackage[pagebackref=true,breaklinks=true,colorlinks]{hyperref}
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{xcolor}

% \let\labelindent\relax
% \usepackage{enumitem}
% \usepackage{xspace}

% %\usepackage{soul}
% %\usepackage{cite}
% \usepackage{makecell}
% \usepackage{multicol}
% \usepackage{rotating}
% \usepackage[percent]{overpic}
% %\usepackage{ulem}

% \usepackage{microtype}
% \usepackage{contour}
% \usepackage{courier}

% \usepackage{subcaption} % issues a warning with CVPR/ICCV format
% \usepackage[font=small]{caption}
% \usepackage[percent]{overpic}
